HawkI: Homography & Mutual Information Guidance for 3D-free Single Image to Aerial View

We present HawkI, for synthesizing aerial-view images from text and an exemplar image, without any additional multi-view or 3D information for finetuning or at inference. HawkI uses techniques from classical computer vision and information theory. It seamlessly blends the visual features from the input image within a pretrained text-to-2Dimage stable diffusion model with a test-time optimization process for a careful bias-variance trade-off, which uses an Inverse Perspective Mapping (IPM) homography transformation to provide subtle cues for aerialview synthesis. At inference, HawkI employs a unique mutual information guidance formulation to steer the generated image towards faithfully replicating the semantic details of the input-image, while maintaining a realistic aerial perspective. Mutual information guidance maximizes the semantic consistency between the generated image and the input image, without enforcing pixel-level correspondence between vastly different viewpoints. Through extensive qualitative and quantitative comparisons against text + exemplar-image based methods and 3D/ multi-view based novel-view synthesis methods on proposed synthetic and real datasets, we demonstrate that our method achieves a significantly better bias-variance trade-off towards generating high fidelity aerial-view images.Code and data is available at https://github.com/divyakraman/HawkI2024.

==> Sections/6-supp_arxiv.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.7]{Figures/supp/syn1.jpg}
    \caption{We show more examples for comparisons with the state-of-the-art image editing, personalization and text-controlled aerial view synthesis methods on the \model-Syn dataset. Our methods is able to generate images that are ``more aerial'', while preserving the fidelity w.r.t. the input image.}
    \label{fig:supp_syn1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.7]{Figures/supp/syn2.jpg}
    \caption{We show more examples for comparisons with the state-of-the-art image editing, personalization and text-controlled aerial view synthesis methods on the \model-Syn dataset. Our methods is able to generate images that are ``more aerial'', while preserving the fidelity w.r.t. the input image.}
    \label{fig:supp_syn1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.7]{Figures/supp/syn3.jpg}
    \caption{We show more examples for comparisons with the state-of-the-art image editing, personalization and text-controlled aerial view synthesis methods on the \model-Syn dataset. Our methods is able to generate images that are ``more aerial'', while preserving the fidelity w.r.t. the input image.}
    \label{fig:supp_syn1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.7]{Figures/supp/syn4.jpg}
    \caption{We show more examples for comparisons with the state-of-the-art image editing, personalization and text-controlled aerial view synthesis methods on the \model-Syn dataset. Our methods is able to generate images that are ``more aerial'', while preserving the fidelity w.r.t. the input image.}
    \label{fig:supp_syn1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.7]{Figures/supp/real1.jpg}
    \caption{We show more examples for comparisons with the state-of-the-art image editing, personalization and text-controlled aerial view synthesis methods on the \model-Real dataset. Our methods is able to generate images that are ``more aerial'', while preserving the fidelity w.r.t. the input image.}
    \label{fig:supp_real1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.7]{Figures/supp/real2.jpg}
    \caption{We show more examples for comparisons with the state-of-the-art image editing, personalization and text-controlled aerial view synthesis methods on the \model-Real dataset. Our methods is able to generate images that are ``more aerial'', while preserving the fidelity w.r.t. the input image.}
    \label{fig:supp_syn1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.7]{Figures/supp/real3.jpg}
    \caption{We show more examples for comparisons with the state-of-the-art image editing, personalization and text-controlled aerial view synthesis methods on the \model-Real dataset. Our methods is able to generate images that are ``more aerial'', while preserving the fidelity w.r.t. the input image.}
    \label{fig:supp_syn1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{Figures/supp/mi_ablations1.jpg}
    \caption{We show a few examples for comparisons with other metrics for diffusion guidance such as L2 distance and Wasserstein distance. Our mutual information guidance method is better at preserving the fidelity w.r.t the input image, as also evidenced by higher SSCD scores. The SSCD score for Wasserstein guidance, $L2$ guidance, and mutual information guidance are $0.3181$, $0.3224$ and $0.3345$ respectively, averaged over all images in the \model-Real dataset.}
    \label{fig:supp_miablation1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{Figures/supp/supp_ablations1.jpg}
    \caption{More qualitative results for ablation experiments.}
    \label{fig:supp_ablation1}
\end{figure*}

\input{Tables/ablations-quant}

\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{Figures/supp/nvs_syn1.jpg}
    \caption{We compare with latest related work on novel view synthesis: Zero-1-to-3 and Zero123++ on images from \model-Syn. Both of these methods use the pretrained stable diffusion model and the 3D objects dataset, Objaverse with 800k+ 3D objects, for training. Our method uses just the pretrained stable diffusion model for the task of aerial view synthesis from a single image.}
    \label{fig:nvs_syn1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.6]{Figures/supp/nvs_real1.jpg}
    \caption{We compare with latest related work on novel view synthesis: Zero-1-to-3 and Zero123++ on images from \model-Real. Both of these methods use the pretrained stable diffusion model and the 3D objects dataset, Objaverse with 800k+ 3D objects, for training. Our method uses just the pretrained stable diffusion model for the task of aerial view synthesis from a single image. 
    \\
    3D generation methods like Zero123++ are capable of generating different views with high fidelity by using pretrained stable diffusion models to finetune on large-scale 3D objects datasets. However, their generalization capabilities are limited. Our method is able to generate high quality aerial images for the given input images without any 3D data and using just the pretrained text-to-2D image stable diffusion model, however, there is scope for improving the fidelity of the generated aerial image w.r.t the input image. Moreover, our method controls the viewpoint via text and does not provide the provision to quantitatively control the camera angle. Both of these limitations of our method can be alleviated by exploring the combination of pretrained Zero123++ models (or other 3D models) and our method, as a part of future work. }
    \label{fig:nvs_real1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.5]{Figures/supp/supp_multiview1.jpg}
    \vspace*{-1em}
    \caption{Additional results on extending \model~to generate other text-controlled views.}
    \label{fig:multiview}
    \vspace*{-0.5em}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.55]{Figures/supp/dataaug1.jpg}
    \caption{\textbf{Can any data augmentation be used in place of Inverse Perspective Mapping (IPM)?} One question that arises from the usage of Inverse Perspective Mapping is related to whether it actually provides pseudo weak guidance, in addition to increasing variance (or reducing bias) in the representation space that is being conditioned for aerial view generation. The latter can be achieved with any random data augmentation. To understand this, we use a $45$ degrees rotated image in place of the image corresponding to the Inverse Perspective Mapping in the second stage of finetuning the text embedding and the diffusion UNet. We do not use mutual information guidance in any of our experiments. Our finding is that results with models that use Inverse Perspective Mapping are generally better in terms of the viewpoint being aerial, while preserving the fidelity with respect to the input image, than models that use the $45$ degree rotated image. Thus, we conclude that rather than using any random data augmentation technique, it is beneficial to use IPM as it is capable of providing pseudo weak guidance to the model for aerial view synthesis. This finding also paves direction for future work on using carefully crafted homography priors for view synthesis corresponding to different camera angles and viewpoints. }
    \label{fig:nvs_real1}
\end{figure*}


